Belief Propagation as Diffusion

We introduce novel belief propagation algorithms to estimate the marginals of a high dimensional probability distribution. They involve natural (co)homological constructions relevant for a localised description of statistical systems.

==> conf/_foldexpr <==
:set foldexpr=getline(v:lnum)[0]==\"\\t\"


==> conf/math <==
\DeclareMathOperator{\e}{e}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\SU}{SU}
\DeclareMathOperator{\U}{U}
\newcommand{\utr}{\mathfrak{u}}
\DeclareMathOperator{\Euc}{Euc}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ahd}{ad}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Harm}{Harm}
\DeclareMathOperator{\T}{T}

\DeclareMathOperator*{\colim}{colim}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%%%%%-Ensembles usuels-%%%%%

\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\Sph}{\mathbb{S}}

%%%%%-Commandes perso-%%%%%
%produits de dualité:
\newcommand\croc[2]{\langle \,#1 \,| \,  #2\, \rangle}
\newcommand\Croc[2]{\big\langle \,#1 \, \big| \,  #2\, \big\rangle}
\newcommand\scal[2]{( #1 \, , \, #2 )}
\newcommand\braket[2]{\langle\, #1 \,| \,  #2\, \rangle}
\newcommand\braaket[3]{\langle\, #1 \,|\, #2 \,|\, #3 \,\rangle}

%somme orthogonale:
\newcommand\Oplus{\overset{\perp}{\oplus}}

%dimensions
\DeclareMathOperator{\Dim}{dim}
\DeclareMathOperator{\Codim}{codim}


==> conf/math.tex <==
\DeclareMathOperator{\e}{e}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\SO}{SO}
\DeclareMathOperator{\SU}{SU}
\DeclareMathOperator{\U}{U}
\newcommand{\utr}{\mathfrak{u}}
\DeclareMathOperator{\Euc}{Euc}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ahd}{ad}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Harm}{Harm}
\DeclareMathOperator{\T}{T}

\DeclareMathOperator*{\colim}{colim}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%%%%%-Ensembles usuels-%%%%%

\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\Sph}{\mathbb{S}}

%%%%%-Commandes perso-%%%%%
%produits de dualité:
\newcommand\croc[2]{\langle \,#1 \,| \,  #2\, \rangle}
\newcommand\Croc[2]{\big\langle \,#1 \, \big| \,  #2\, \big\rangle}
\newcommand\scal[2]{( #1 \, , \, #2 )}
%\newcommand\braket[2]{\langle\, #1 \,| \,  #2\, \rangle}
%\newcommand\braaket[3]{\langle\, #1 \,|\, #2 \,|\, #3 \,\rangle}

%somme orthogonale:
\newcommand\Oplus{\overset{\perp}{\oplus}}

%dimensions
\DeclareMathOperator{\Dim}{dim}
\DeclareMathOperator{\Codim}{codim}

